Featured Team Automata

We propose featured team automata to support variability in the development and analysis of teams, which are systems of reactive components that communicate according to specified synchronisation types. A featured team automaton concisely describes a family of concrete product models for specific configurations determined by feature selection. We focus on the analysis of communication-safety properties, but doing so product-wise quickly becomes impractical. Therefore, we investigate how to lift notions of receptiveness (no message loss) to the level of family models. We show that featured (weak) receptiveness of featured team automata characterises (weak) receptiveness for all product instantiations. A prototypical tool supports the developed theory.

==> src/img/feta-with-req.tex <==
% !TEX root=featured-team.tex

\begin{tikzpicture}[align=center, every node/.style={scale=.9,font=\footnotesize}]
  % states
  \node[rloc](000){$0,0,0$};
  \node[rloc,right=5 of 000](020){$0,2,0$};
  \coordinate(mid1) at ($(000)!.5!(020)$);
  \node[rloc,above=1 of mid1](011){$0,1,1$};
  \node[rloc,below=4 of 000](200){$2,0,0$};
  \node[rloc,below=4 of 020](220){$2,2,0$};
  \coordinate(mid2) at ($(200)!.5!(220)$);
  \node[rloc,below=1 of mid2](211){$2,1,1$};
  \coordinate(mid3) at ($(020)!.5!(220)$);
  \node[rloc,right=1 of mid3](121){$1,2,1$};
  \coordinate(mid4) at ($(000)!.5!(200)$);
  \node[rloc,left=1 of mid4](101){$1,0,1$};
  % transitions
  \path[->] 
    (000) edge[bend left=10,above] node{\trFe{\unlock[]}\Label{u_2}{join}{s}} (020)
    (000) edge[bend left=10,above,sloped] node{\trFe{\lock[]}\Label{u_2}{join}{s}} (011)
    (000) edge[bend right=10,above,sloped] node[yshift=8pt]{\trFe{\lock[]}\Label{u_1}{join}{s}} (101)
    (000) edge[bend left=10,above, sloped ] node{\trFe{\unlock[]}\Label{u_1}{join}{s}} (200)
    (000) edge[bend left=10,above, sloped ] node{\trFe{\unlock[]}\Label{u_1,u_2}{join}{s}} (220)
    (011) edge[bend left=10,above, sloped] node{\trFe{\lock[]}\Label{s}{confirm}{u_2}} (020)
    (020) edge[bend left=10,above] node{\trFe{\lock[]\xor \unlock[]}\Label{u_2}{leave}{s}} (000)
    (020) edge[bend left=10,above,sloped] node[yshift=8pt]{\trFe{\lock[]}\Label{u_1}{join}{s}} (121)
    (020) edge[bend left=10,above,sloped] node{\trFe{\unlock[]}\Label{u_1}{join}{s}} (220)
    (121) edge[bend left=10,below, sloped] node[yshift=-8pt]{\trFe{\lock[]}\Label{s}{confirm}{u_1}} (220)
    (220) edge[bend left=10,above] node{\trFe{\lock[]\xor \unlock[]}\Label{u_2}{leave}{s}} (200)
    (200) edge[bend left=10,above] node{\trFe{\unlock[]}\Label{u_2}{join}{s}} (220)
    (200) edge[bend left=10,above,sloped] node{\trFe{\lock[]\xor \unlock[]}\Label{u_1}{leave}{s}} (000)
    (200) edge[bend right=10,below,sloped] node{\trFe{\lock[]}\Label{u_2}{join}{s}} (211)
    (220) edge[bend left=10,above, sloped] node{\trFe{\lock[]}\Label{u_1,u_2}{leave}{s}} (000)
    (220) edge[bend left=10,above,sloped] node{\trFe{\lock[]\xor \unlock[]}\Label{u_1}{leave}{s}} (020)
    (101) edge[bend right=10,below,sloped] node[yshift=-8pt]{\trFe{\lock[]}\Label{s}{confirm}{u_1}} (200)
    (211) edge[bend right=10,below,sloped] node{\trFe{\lock[]}\Label{s}{confirm}{u_2}} (220);
  % initial 
  \coordinate[above=0.3 of 000](initial);
  \draw[->,thick] (initial) -> (000);
    % fm 
    \node[below=2 of 211] (fm) {$\fm = \Fe{\lock\xor \unlock}$};
    % requirements 
    \node[req,above=0.8 of 000,xshift=-1cm](r000){
      \Req{\bigwedge_{i\in\{1,2\}}(u_i,\mi{join})_\Fe{\lock\xor \unlock}\land\\
       (\{u_1,u_2\},\mi{join})_\Fe{\lock \land \neg \unlock}
       }{(s,\mi{join})_\Fe{\lock\xor \unlock}\lor(s,leave)_\Fe{\lock\xor \unlock}}
    }; 
    \node[req,above=0.8 of 020,xshift=1cm](r020){
      \Req{(u_1,\mi{join})_\Fe{\lock\xor \unlock}\land(u_2,\mi{leave})_\Fe{\lock\xor \unlock}
      }{(s,\mi{join})_\Fe{\lock\xor \unlock}\lor(s,\mi{leave})_\Fe{\lock\xor \unlock}}
    };
    \node[req,above=0.5 of 011](r011){
      \Req{(u_1,\mi{join})_\Fe{\lock\xor \unlock}\land\\(s,\mi{confirm})_\Fe{\lock\land\neg \unlock}}{}
    };
    \node[req,below=0.5 of 211](r211){
      \Req{(u_1,\mi{leave})_\Fe{\lock\xor \unlock}\land\\(s,\mi{confirm})_\Fe{\lock\land\neg\unlock}}{}
    };
    \node[req,below=1 of 220,xshift=20pt](r220){
      \Req{\bigwedge_{i\in\{1,2\}}(u_i,\mi{leave})_\Fe{\lock\xor \unlock}\land\\
      (\{u_1,u_2\},\mi{leave})_\Fe{\lock\xor \unlock}}{
      (s,\mi{leave})_\Fe{\lock\xor \unlock}\lor(s,\mi{join})_\Fe{\lock\xor \unlock}}
    };
    \node[req,below=1 of 200,xshift=-20pt](r200){
      \Req{(u_1,\mi{leave})_\Fe{\lock\xor \unlock}\land
    (u_2,\mi{join})_\Fe{\lock\xor \unlock}}{
    (s,\mi{leave})_\Fe{\lock\xor \unlock}\lor(s,\mi{join})_\Fe{\lock\xor \unlock}}
    };
    \node[req,above=1.7 of 101,xshift=-25pt](r101){
      \Req{(u_2,\mi{join})_\Fe{\lock\xor \unlock}\land\\(s,\mi{confirm})_\Fe{\lock\land\neg\unlock}}{}
    };
    \node[req,above=1.7 of 121,xshift=25pt](r121){
      \Req{(u_2,\mi{leave})_\Fe{\lock\xor \unlock}\land\\(s,\mi{confirm})_\Fe{\lock\land\neg\unlock}}{}
    };
    % requirements links
    \path[-,dotted] 
    (000) edge[bend left=10] (r000)
    (020) edge[bend right=10] (r020)
    (011) edge[bend right=0] (r011)
    (101) edge[bend left=30] (r101)
    (220) edge[bend left=10] (r220)
    (211) edge[bend left=0] (r211)
    (200) edge[bend right=10] (r200)
    (121) edge[bend right=30] (r121);
\end{tikzpicture}

==> src/preamble.tex <==
% !TEX root=featured-team.tex
\usepackage{graphicx}
\usepackage{graphics}
\usepackage[pdf]{graphviz}
% \usepackage{amsthm}
% \usepackage{amsmath}
\usepackage{mathrsfs}
\usepackage{mathtools}
\usepackage{amsfonts}
\usepackage{float}
\usepackage{amssymb}
\usepackage{stmaryrd}
\SetSymbolFont{stmry}{bold}{U}{stmry}{m}{n}
\usepackage{bm}
\usepackage{dsfont}
\usepackage{xspace}
\usepackage[normalem]{ulem}
\usepackage[dvipsnames]{xcolor}
%\usepackage[colorlinks=true]{hyperref}
%\hypersetup{%
%  colorlinks  = true,
%  linkcolor   = blue!75!black,
%  citecolor   = blue!75!black,
%  urlcolor    = blue!80
%}
% For Springer
\makeatletter
\RequirePackage[bookmarks,unicode,colorlinks=true]{hyperref}%
   \def\@citecolor{blue}%
   \def\@urlcolor{blue}%
   \def\@linkcolor{blue}%
\def\UrlFont{\rmfamily}
\def\orcidID#1{\smash{\href{http://orcid.org/#1}{\protect\raisebox{-1.25pt}{\protect\includegraphics{src/img/orcid_color-eps-converted-to.pdf}}}}}
\makeatother
\usepackage[nameinlink,capitalise]{cleveref}
\usepackage{url}
\usepackage{booktabs}
\usepackage[inline]{enumitem}
\usepackage[linesnumbered,lined,commentsnumbered,noend,vlined,ruled]{algorithm2e} %,boxed
\usepackage{longtable}
\usepackage{multirow}
\usepackage{footnote}
\usepackage{listings}
\usepackage{bold-extra}
\usepackage{relsize}
\usepackage[scaled=0.85]{beramono}
%% Only if the base font of the document is to be typewriter style
\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}
\usepackage{tikz-cd}
\usepackage{tikz}
\usetikzlibrary{arrows,calc,shapes.arrows,shapes.multipart,shapes.geometric, positioning, shadows, automata,fit,decorations.markings,decorations.pathmorphing,backgrounds}
\usepackage{wasysym}
\usepackage{fontawesome}
\usepackage{caption}
\usepackage{subcaption}
\makeatletter
\providecommand{\leftsquigarrow}{%
  \mathrel{\mathpalette\reflect@squig\relax}%
}
\newcommand{\reflect@squig}[2]{%
  \reflectbox{$\m@th#1\rightsquigarrow$}%
}
\makeatother
\usepackage{thm-restate}

% environments
\newenvironment{myfigure}{\begin{figure}[tb]}{\end{figure}}
% \newtheorem{definition}{Definition}
% \newtheorem{example}{Example}
\newcommand{\myparagraph}[1]{\medskip\noindent\textbf{#1} }
\newcommand{\mysparagraph}[1]{\smallskip\noindent\textbf{#1} }
\newcommand{\wrap}[1]{\begin{tabular}{@{}c@{}}#1\end{tabular}}
\newcommand{\lwrap}[1]{\begin{tabular}{@{}l@{}}#1\end{tabular}}
\newcommand{\mwrap}[1]{\begin{array}{@{}c@{}}#1\end{array}}
\newcommand{\mlwrap}[1]{\begin{array}{@{}l@{}}#1\end{array}}
\newcommand{\mytikz}[1]{\wrap{\begin{tikzpicture}[align=center]#1\end{tikzpicture}}}

% colors
\definecolor{dblue}{RGB}{52, 81, 105}
\definecolor{lblue}{RGB}{218, 218, 247}
\definecolor{webgreen}{rgb}{0,.5,0}
\definecolor{webbrown}{rgb}{.6,0,0}
\definecolor{myred}{rgb}{.7,0,0}
\definecolor{mypurple}{rgb}{.5,0,0.6}
\definecolor{mypurple2}{HTML}{800080}
\definecolor{dslcomments}{HTML}{308495}%3089B6

% tikz
\tikzstyle{loc}=[draw=black,circle,rounded corners=5pt,inner sep=3pt]
\tikzstyle{rloc}=[draw=black,rectangle,rounded corners=5pt,inner sep=3pt]
  % minimum width=3.2em, minimum height=1.45em]
\tikzstyle{req}=[ rectangle split,
       rectangle split parts=1,%2,
       rectangle split part fill={myorange!20,myorange!20},
       rounded corners=1pt,
       draw=black, 
       dotted,
       minimum height=1em,
       % text width=3cm,
       inner sep=2pt,
       text centered]
\tikzstyle{eloc}=[ rectangle split,
       rectangle split parts=3,
       fill=myorange!20,
       rounded corners=1pt,
       draw=black, 
       dotted,
       minimum height=1em,
       % text width=3cm,
       inner sep=2pt,
       text centered]       
\tikzstyle{myinit}=[loc,double,inner sep=4pt] % accepting,state
\tikzstyle{lb}=[pos=1,inner sep=0]
\tikzstyle{mynode}=[fill=red!20,circle,inner sep=0pt,draw]
\tikzstyle{myQ}=[fill=yellow!20, rectangle split, rectangle split parts=3, 
                draw, rectangle split horizontal, 
                rectangle split part align={center, top, bottom}]
\tikzstyle{myarrow}=[fill=red!50, single arrow, draw]
\tikzstyle{myCBQ}=[fill=green!10, draw, minimum height=1.5em, minimum width=3.5em, 
                  double copy shadow={shadow xshift=4pt, shadow yshift=4pt, 
                  fill=green!10, draw}]
\tikzstyle{bx}=[draw=black,inner sep=2.5mm,thick,minimum height=10mm
                ,rounded corners=3pt,font=\footnotesize]
\tikzstyle{pr}=[circle,draw=black,very thick,fill=white,inner sep=2pt]
\tikzstyle{lbl}=[rotate=0,font=\scriptsize]


\tikzstyle{grad}=[draw=dblue,fill=white, postaction={path fading=north, fading angle=45, fill=lblue,draw=dblue}]
\tikzstyle{myhubtkz}=[grad,thick,font={\footnotesize\rm\color{dblue}}]
\tikzstyle{myhublt}=[myhubtkz,minimum height=5mm,inner sep=0.5pt]
\newcommand{\myhub}[2][]{\raisebox{-1.5mm}%
    {\tikz{\node[myhubtkz,#1]{#2};}}}

\definecolor{myblue}{HTML}{617be3}
\definecolor{myorange}{HTML}{e39c61}
\tikzstyle{var}=[circle,draw=black,font=\bf\ttfamily\footnotesize
                ,minimum height=6mm,fill=myorange!50]
\tikzstyle{fun}=[rectangle,draw=black,inner sep=1.5mm,rounded corners=0.5mm
                ,minimum height=1,font=\bf\ttfamily\footnotesize,fill=myblue!50]
\tikzstyle{source}=[var,regular polygon, regular polygon sides=3,inner sep=2pt]
\tikzstyle{sourcef}=[var,regular polygon, regular polygon sides=3,inner sep=0pt,minimum width=23pt]
\tikzstyle{sourceonce}=[sourcef,ultra thick]
\tikzstyle{sink}=[var,regular polygon, rectangle]
\tikzstyle{arr}=[->,rounded corners=5pt,>=stealth']

% I.e.
\newcommand{\ie}{I.e.\xspace}
% e.g.,
\newcommand{\eg}{e.g.,\xspace}
% mathscr 
\newcommand{\fancy}[1]{\ensuremath{\mathcal{#1}}\xspace}
% projection 
\newcommand{\proj}{{\ensuremath{\downharpoonright}\xspace}}
% allow break
\newcommand{\ab}{\allowbreak}
% mathit
\newcommand{\mi}[1]{\ensuremath{\mathit{#1}}\xspace}

% automata helpers
\newcommand{\autNameTxt}[1]{\textcolor{red!20!black}{\mii{#1}}\xspace}
\newcommand{\autName}[1]{\autNameTxt{{\scriptsize{#1}}\xspace}}
\newcommand{\nodeName}[1]{\textcolor{red!50!black}{\mi{#1}}\xspace}
\newcommand{\nodeInv}[1]{\textcolor{violet}{\mi{#1}}\xspace}
\newcommand{\trGuard}[1]{\mi{\big\langle \textcolor{green!50!black}{#1}\big\rangle}}
\newcommand{\trAct}[1]{\textcolor{blue!90!black}{\mathsf{#1}}\xspace}
\newcommand{\trUpd}[1]{\textcolor{blue!30!black}{\mi{#1}}\xspace}
\newcommand{\myParam}[1]{\textcolor{red}{\textsf{\scriptsize{#1}}}\xspace}
\newcommand{\myVar}[1]{\textcolor{black}{\textsf{\scriptsize{#1}}}\xspace}
% \newcommand{\trFe}[1]{\mi{[\textcolor{black}{#1}]}}
\newcommand{\trFe}[1]{\mi{[\textcolor{green!45!black}{#1}]}}
% \newcommand{\Fe}[1]{\mi{\textcolor{green!50!black}{#1}}}
\newcommand{\Fe}[1]{\mi{#1}}
\newcommand{\trFeTxt}[1]{\ensuremath{\mathit{\textcolor{green!50!black}{#1}}}\xspace}
\newcommand{\nodeNameTxt}[1]{\textcolor{red!50!black}{\ensuremath{\mathit{#1}}}\xspace}
\newcommand{\nodeInvTxt}[1]{\textcolor{violet}{\ensuremath{\mathit{#1}}}\xspace}
\newcommand{\trGuardTxt}[1]{\ensuremath{\mathit{\textcolor{green!50!black}{#1}}}\xspace}
\newcommand{\trActTxt}[1]{\textcolor{blue!90!black}{\ensuremath{\mathit{#1}}}\xspace}
\newcommand{\trUpdTxt}[1]{\textcolor{blue!30!black}{\ensuremath{\mathit{#1}}}\xspace}
\newcommand{\myParamTxt}[1]{\textcolor{red}{\ensuremath{\mathit{\textsf{#1}}}}\xspace}
\newcommand{\myVarTxt}[1]{\textcolor{black}{\ensuremath{\mathit{\textsf{#1}}}}\xspace}
% transition
\newcommand{\tr}[1]{\xrightarrow{\xspace{#1}\xspace}}
\newcommand{\ttr}[2][]{\xrightarrow[#1]{#2}}

% semantics
\newcommand{\sem}[1]{\ensuremath{{\left\llbracket#1\right\rrbracket}}}
% set
% \newcommand{\set}[1]{\left\{#1\right\}}
\newcommand{\set}[1]{\{#1\}}
% tuple
\newcommand{\tpl}[1]{\ensuremath{\langle #1 \rangle}\xspace}
% overline
\newcommand{\ol}[1]{\ensuremath{\overline{#1}}}
% underline
\newcommand{\ul}[1]{\ensuremath{\underline{#1}}}
% power set
\newcommand{\pset}[1]{\ensuremath{\bkw{2}^{#1}}}

\newcommand{\Nat}{\ensuremath{\mathbb{N}}\xspace}
\newcommand{\Bool}{\ensuremath{\mathbb{B}}\xspace}
\newcommand{\I}{\ensuremath{\mathcal{I}}\xspace}
\newcommand{\T}{\ensuremath{\mathcal{T}}\xspace}
\newcommand{\A}{\ensuremath{\mathcal{A}}\xspace}
% \newcommand{\TS}{\ensuremath{\mathcal{T}\!\mathcal{S}}\xspace}
\newcommand{\GG}{\ensuremath{\mathcal{G}}\xspace}
\newcommand{\B}{\ensuremath{\mathcal{B}}\xspace}
\newcommand{\D}{\ensuremath{\mathcal{D}}\xspace}
\renewcommand{\P}{\ensuremath{\mathcal{P}}\xspace}
\newcommand{\W}{\ensuremath{\mathcal{W}}\xspace}
\newcommand{\F}{\ensuremath{\mathcal{F}}\xspace}
\renewcommand{\L}{\ensuremath{\mathcal{L}}\xspace}
\newcommand{\mbb}[1]{\ensuremath{\mathbb{#1}}}
% keywords
\newcommand{\kw}[1]{{\textsf{\upshape #1}}}
% bold keywords
\newcommand{\bkw}[1]{\textbf{\kw{#1}}}
% quotes in math
\newcommand{\mquote}[1]{\text{`\ensuremath{#1}'}}
% vertical bold bar
\newcommand{\vbar}{\raisebox{-3.5pt}{\tikz{\draw[very thick] (0,0) -- (0,.45)}}\xspace}
% condition with left {
\newcommand{\ifcond}[1]{\left\{\begin{array}{l@{}}#1\end{array}\right.}

\newcommand{\nline}{\\[0pt]}
% mathcal
\newcommand{\mc}[1]{\ensuremath{\mathcal{#1}}\xspace}

%%%%%%% adding comments %%%%%%%%%%%%%%%%%%%%%%%
\usepackage[normalem]{ulem}
\usepackage[textwidth=39.0mm,textsize=scriptsize]{todonotes}
% \setlength{\evensidemargin}{13.3mm}
\setlength{\marginparwidth}{39.0mm}
\newcommand{\bgtext}[1]{%
  \bgroup\markoverwith {\textcolor{#1}{\rule[-0.5ex]{2pt}{11pt}}}\ULon}
\newcommand{\mytodon}[2]{\noindent\todo[color=#1,tickmarkheight=1mm]{#2}}
\newcommand{\josetodo}[2][]{\bgtext{red!25   }{#1}\mytodon{red!50}{J: #2}}
\newcommand{\guilletodo}[2][]{\bgtext{blue!20}{#1}\mytodon{blue!40}{G: #2}}
\newcommand{\mautodo}[2][]{\bgtext{orange!25}{#1}\mytodon{orange!50}{M: #2}}
\newcommand{\rolftodo}[2][]{\bgtext{green!25}{#1}\mytodon{green!50}{R: #2}}
% \newcommand{\josein}[2][\textwidth]{
%   \mytodon{red!50,inline,inlinewidth=#1,noinlinepar}{José: #2}}
% \newcommand{\guillein}[2][\textwidth]{
%   \mytodon{blue!40,inline,inlinewidth=#1,noinlinepar}{Guille: #2}}
%
\newcommand{\mytodo}[2]{\textcolor{#1}{===#2}}
\newcommand{\jose}[1]{\mytodo{red!75!black}{José: #1}}
\newcommand{\guille}[1]{\mytodo{blue!75!black}{Guille: #1}}
\newcommand{\rolf}[1]{\mytodo{green!55!black}{Rolf: #1}}
\newcommand{\mau}[1]{\mytodo{orange!75!black}{Mau: #1}}

% \renewcommand{\mytodo}[2]{}
% \renewcommand{\mytodon}[2]{}

%%

% syntax highlight box
\newcommand{\shl}[2][gray]{{\setlength\fboxsep{2pt}\colorbox{#1!20}{{#2}}\setlength\fboxsep{2pt}}}
% syntax highlight box in math
\newcommand{\mshl}[2][gray]{\shl[#1]{\ensuremath{#2}}\xspace}
% texttt
\newcommand{\stt}[1]{{\small\texttt{#1}}\xspace}

% features
\newcommand{\fm}{\mi{fm}}
\newcommand{\FE}{\mi{FE}}
\newcommand{\fe}[1]{{\mshl{_{\bkw{fe}#1}}}}
\newcommand{\verum}{\ensuremath{\mathord{\bm{\top}}}\xspace}
\newcommand{\falsum}{\ensuremath{\mathord{\bm{\perp}}}\xspace}
\newcommand{\xor}{\oplus}
\newcommand{\nand}{\uparrow}
\newcommand{\FETA}{f\ensuremath{\mkern1mu}ETA\xspace}
\newcommand{\FTS}{f\ensuremath{\mkern1mu}TS\xspace}
\newcommand{\FSTS}{f\ensuremath{\mkern1mu}STS\xspace}
\newcommand{\FSys}{f\ensuremath{\mkern1mu}Sys\xspace}
\newcommand{\FCA}{f\ensuremath{\mkern1mu}CA\xspace}
\newcommand{\FREQ}{f\ensuremath{\mkern1mu}Req\xspace}
\newcommand{\mFETA}{\ensuremath{\mathit{fETA}}\xspace}
\newcommand{\mFTS}{\ensuremath{\mathit{fTS}}\xspace}
\newcommand{\mFSTS}{\ensuremath{\mathit{fSTS}}\xspace}
\newcommand{\mFSys}{\ensuremath{\mathit{fSys}}\xspace}
\newcommand{\mFCA}{\ensuremath{\mathit{fCA}}\xspace}
\newcommand{\ETA}{ETA\xspace}
\newcommand{\TS}{TS\xspace}
\newcommand{\LTS}{LTS\xspace}
\newcommand{\STS}{STS\xspace}
\newcommand{\Sys}{system\xspace}
\newcommand{\CA}{CA\xspace}
\newcommand{\REQ}{Req\xspace}
% \newcommand{\FETAs}{f\ensuremath{\mkern1mu}ETAs\xspace}
\newcommand{\FTSs}{f\ensuremath{\mkern1mu}TSs\xspace}
\newcommand{\FSTSs}{f\ensuremath{\mkern1mu}STSs\xspace}
\newcommand{\FSyss}{f\ensuremath{\mkern1mu}Sys's\xspace}
\newcommand{\FREQs}{fReqs\xspace}
\newcommand{\TSs}{TSs\xspace}
\newcommand{\LTSs}{LTSs\xspace}
\newcommand{\STSs}{STSs\xspace}
\newcommand{\Syss}{systems\xspace}
\newcommand{\REQs}{Reqs\xspace}


\newcommand{\lock}[1][\textcolor{black!50}]{\text{#1{\smaller\faLock}}\xspace}
\newcommand{\unlock}[1][\textcolor{black!50}]{\text{#1{\smaller\faUnlock}}\xspace}
% \newcommand{\auth}{\text{\smaller\faKey}\xspace}
\newcommand{\auth}{@}%\newcommand{\auth}{\textit{auth}\xspace} @ stands for access (management system)
\newcommand{\server}{\mathbb S}
\newcommand{\user}{\mathbb U}

% \newcommand{\qedx}{\pushQED{\qed}\renewcommand{\qedsymbol}{$\triangle$}\qed\popQED}
\newcommand\xqed[1]{%
  \leavevmode\unskip\penalty9999 \hbox{}\nobreak\hfill
  \quad\hbox{#1}}
\newcommand\qedx{\xqed{$\vartriangleright$}} % $\triangleright \rhd \vartriangleright$
\newcommand{\qedhere}{\tag*{\qed}}

% ETA 
\newcommand{\N}{\fancy{N}\xspace}
\newcommand{\E}{\fancy{E}\xspace}
\newcommand{\R}{\ensuremath{\mathcal{R}}\xspace}
\renewcommand{\S}{\ensuremath{\mathcal{S}}\xspace}
\newcommand{\FS}{\ensuremath{\mathcal{FS}}\xspace}
\newcommand{\spol}{\ensuremath{\varepsilon}\xspace}
\newcommand{\stype}{\bkw{st}\xspace}
\newcommand{\fstype}{\bkw{fst}\xspace}
\newcommand{\slbl}[1][]{\ensuremath{\Lambda_{{#1}}(\mc{S})}\xspace}
\newcommand{\sys}{\ensuremath{\mc{S}}\xspace}
\newcommand{\rcp}{\bkw{rcp}\xspace}
\newcommand{\rsp}{\bkw{rsp}\xspace}
% \newcommand{\com}{\ensuremath{\Sigma^\bullet}\xspace}
\newcommand{\com}{\ensuremath{\Sigma}\xspace}
\newcommand{\dom}{\ensuremath{\bkw{dom}}\xspace}
\newcommand{\domin}{\ensuremath{\bkw{dom}^?}\xspace}
\newcommand{\domout}{\ensuremath{\bkw{dom}^!}\xspace}
\newcommand{\complies}{\ensuremath{\models\xspace}}
\newcommand{\wcomplies}{\ensuremath{\models^{\scriptstyle\bkw{*}}\xspace}}
% ETA tikz
\newcommand{\Snd}[1]{\ensuremath{\{#1\}}}
\newcommand{\Rec}[1]{\ensuremath{\{#1\}}}
\newcommand{\Label}[3]{\ensuremath{\Snd{#1},\mathit{#2},\Rec{#3}}}
\newcommand{\Req}[2]{\ensuremath{\mlwrap{#1}}}%\nodepart{two}}\ensuremath{\mlwrap{#2}}}
\newcommand{\Node}[3]{%
  \ensuremath{\langle#1\rangle}\nodepart{two}%
  \ensuremath{\mlwrap{#2}}\nodepart{three}%
  \ensuremath{\mlwrap{#3}}}
\newcommand{\Chi}[1]{\raisebox{2pt}{{$\chi$}}\ensuremath{_{#1}}\xspace}

% Logic
%----------------------------------------------------------------------------------------
\newcommand{\Forall}{\forall~}
\newcommand{\Exists}{\exists~}
\newcommand{\Iff}{\Leftrightarrow}
\newcommand{\Implies}{\Rightarrow}

% Figures with numbers
%----------------------------------------------------------------------------------------
\tikzstyle{nitem}=[circle,draw=black,thick,fill=myblue!50,inner sep=1pt] 
\newcommand{\sshot}[2]{
  \includegraphics[scale=#2]{src/img/#1.png}}
\newcommand{\numsshot}[3][0.36]{
\tikz{\node[inner sep=0] (img) {\sshot{#2}{#1}};
  \node[nitem,anchor=north east, xshift = -18pt,yshift=-2pt]at(img.north east) {{#3}};}}
% circle numbered items  
\newcommand{\cn}[1]{\raisebox{-3pt}{\tikz{\node[nitem]{#1}}}}

\hyphenation{re-a-lis-a-ble}

% Spacing:
\setlength{\intextsep}{0.25cm}
\setlength{\abovecaptionskip}{0.2cm}
%\usepackage{setspace}
%\setlength{\intextsep}{4pt}
%\setlength{\abovecaptionskip}{6pt}
%\setlength{\belowcaptionskip}{2pt}
%\setlength{\floatsep}{6pt}
%\setlength{\textfloatsep}{6pt}
%\setlength{\dbltextfloatsep}{0pt}


